Measuring and Exploiting Implicit Trust in LLM Tool-Calling Pipelines

The Model Context Protocol (MCP) enables LLMs to invoke external tools, but every tool interaction exposes the model to attacker-controlled text through multiple input channels (tool descriptions, tool results, sampling messages) that share a single context window without privilege separation. In this paper, we present a framework to measure the trust profile of an arbitrary LLM based on a variety of payload framings sent through different channels. Following this assessment, we devise cross-channel fragmentation attacks that distribute seemingly benign payloads across two or three channels; no individual channel carries a complete injection, yet the LLM compiles the fragments into credential exfiltration. We evaluated our attacks across 12 frontier models, three production clients, and six payloads, totalling over 15,000 trials. Our evaluation reveals that cross-channel attacks are an unexplored attack surface: models that fully resist single-channel injection (0% compliance) exfiltrate sensitive data at up to 100% under two-channel fragmentation (e.g., GPT-4o, Llama 70B, Composer 2, Haiku 4.5). We further demonstrate value-aligned exploitation, where a tool's stated purpose requires the data the attacker targets, and a sampling system prompt override that injects persistent instructions via VS Code's MCP implementation. Finally, we evaluated our attacks against seven third-party MCP security tools and three prompt-based defenses. All tools failed to detect fragmented payloads, and prompt defenses proved model-specific rather than universal.

==> sections/06_related.tex <==
% ============================================================
\section{Related Work}
\label{sec:related-work}

Section~\ref{sec:related} positioned our measurement methodology against prior injection benchmarks (Table~\ref{tab:related}).
Here we situate the broader contributions of this work within three related areas: software supply chain security, prompt injection defenses, and the emerging MCP security tool ecosystem.

% ────────────────────────────────────────────────────────────
\subsection{Software Supply Chain Attacks}

Package manager poisoning is a well-studied attack class in which an attacker publishes a malicious package (npm, PyPI, RubyGems) that developers install as a trusted dependency.
MCP servers follow the same installation trust model: a developer adds a server through a configuration file, the server runs as a local process with the developer's filesystem permissions, and its behavior is not audited after installation.
OX Security~\cite{oxsecurity2026mcp} demonstrated that 9 of 11 public MCP registries accepted a malicious proof-of-concept server, confirming that the registry layer provides no meaningful barrier to publication.

MCP servers differ from npm packages in two respects that favor the attacker.
First, an npm package's behavior is fixed at install time and auditable through source review; an MCP server can change its tool descriptions and tool results between invocations without any update notification (OpenClaw, CVE-2026-32979).
Second, npm packages do not receive the contents of \texttt{.env} files and SSH private keys as function arguments from the runtime; MCP tool calls do, because the LLM reads files and passes them as parameters at the model's own initiative.
Schneier~\cite{schneier2026promptware} frames this class of adversarial LLM inputs as ``promptware,'' a new software attack class where traditional input validation fails because the input is natural language processed by a statistical model.

% ────────────────────────────────────────────────────────────
\subsection{Prompt Injection Defenses}

Defenses against prompt injection fall into three categories.

\emph{Input-level defenses} attempt to separate trusted from untrusted content before it reaches the model.
StruQ~\cite{chen2024struq} encodes the distinction structurally by using separate token sequences for instructions versus data.
The instruction hierarchy~\cite{wallace2024instruction} trains models to assign privilege levels to input sources (system $>$ user $>$ tool).
Both assume a fixed channel ordering, which our trust hierarchy measurements show is model-specific: enforcing ``system $>$ tool'' increases exposure on models where \channel{System} is already the most compliant channel (\S\ref{sec:prompt-defenses}).

\emph{Architectural defenses} remove untrusted content from the generation context entirely.
CaMeL~\cite{camel2025} separates code generation from data processing using a dual-LLM architecture, preventing tool-result content from influencing code generation.
This addresses the root cause of cross-channel fragmentation but introduces utility tradeoffs and is not implemented in any production MCP client.

\emph{Detection-based defenses} classify inputs as benign or malicious at runtime.
Invariant Guardrails~\cite{invariant2025github} applies an ML-based prompt injection detector to tool results.
Pipelock~\cite{pipelock2026} uses regex-based pattern matching on both tool descriptions and tool results.
Trail of Bits~\cite{trailofbits2025mcp} applies TOFU pinning to tool descriptions and an optional local classifier to tool results.
Our evaluation in \S\ref{sec:deployed-tools} shows that detection-based defenses catch direct injection payloads but miss compliance-framed payloads (SOC-2, FC) and all fragmented payloads.

Nasr et al.~\cite{nasr2025attacker} formalize the observation that adaptive attackers bypass most proposed defenses, establishing that static defense evaluation understates real-world risk.
Our work provides empirical evidence for this claim: the most capable runtime defense (Pipelock) blocks all 6 direct payloads but is bypassed by substituting a single verb in the fragmented variant.

% ────────────────────────────────────────────────────────────
\subsection{MCP Security Ecosystem}

The MCP security tool ecosystem has grown rapidly since mid-2025.
Four static scanners (Tencent AI-Infra-Guard~\cite{tencent2026aig}, Snyk agent-scan~\cite{snyk2026agentscan}, Agentic Radar~\cite{agenticradar2026}, Cisco MCP Scanner~\cite{ciscomcp2026}) analyze tool descriptions at install time.
Three runtime tools (Invariant~\cite{invariant2025github}, Pipelock~\cite{pipelock2026}, Trail of Bits~\cite{trailofbits2025mcp}) inspect tool results or enforce configuration integrity during execution.
The OWASP MCP Top~10~\cite{owasp2025mcp} identifies tool poisoning and rug pulls as top risks but provides no per-channel empirical data.
Docker Labs~\cite{docker2025whatsapp} demonstrated MCP-based WhatsApp data exfiltration as a proof of concept without systematic measurement.

Our work differs from the tool ecosystem in scope: we do not propose a new scanner but instead measure the attack surface that all existing scanners must cover.
The trust hierarchy (\S\ref{sec:1ch-results}) and fragmentation bypass (\S\ref{sec:frag-results}) provide a benchmark against which future MCP defense tools can be evaluated.


==> sections/07_ethics.tex <==
%\noindent\textbf{Ethics and Disclosure:} 
\section*{Ethics and Disclosure}
We have responsibly disclosed all
our findings to \revised{the affected vendors (OpenAI, Microsoft, Anthropic, and Google), while their investigations are}
pending. No attacks were launched on external hosts and only
synthetic credentials were used in our experiments.
\revised{No human subjects were involved; all trials targeted LLM
APIs and locally installed MCP clients under our control.}

